On the performance of the variational multiscale formulation for subsurface flow and transport in heterogeneous porous media

The following work compares two popular mixed finite elements used to model subsurface flow and transport in heterogeneous porous media; the lowest order Raviart-Thomas element and the variational multiscale stabilized element. Comparison is made based on performance for several problems of engineering relevance that involve highly heterogenous material properties (permeability ratios of up to $1\times10^5$), open flow boundary conditions (pressure driven flows), and large scale domains in two dimensions. Numerical experiments are performed to show the degree to which mass conservation is violated when a flow field computed using either element is used as the advection velocity in a transport model. The results reveal that the variational multiscale element shows considerable mass production or loss for problems that involve flow tangential to layers of differing permeability, but marginal violation of local mass balance for problems of less orthogonality in the permeability. The results are useful in establishing rudimentary estimates of the error produced by using the variational mutliscale element for several different types of problems.

==> Sections/PF_Figures.tex <==
%********************************************;
%                                            ;
%  NAME                                      ;
%    Figures.tex                             ;
%                                            ;
%  WRITTEN BY                                ;
%    Daniel Turner                           ;
%                                            ;
%********************************************;

% \section*{}
%
\begin{figure}[htb!]
	\centering
 \includegraphics[scale=0.40]{./Figures/Elements.pdf}
	\caption{The left figure shows the degrees-of-freedom in the lowest-order 
	Raviart-Thomas (RT0) formulation, and the right figure shows the 
	degrees-of-freedom in the (equal-order) VMS formulation.}
	\label{fig:Elements}
\end{figure}
%
\begin{figure}[htb!]
	\centering
 \subfigure{\includegraphics[scale=0.55]{./Figures/Layers_Geo.pdf}}
 \subfigure{ \includegraphics[scale=0.30]{./Figures/Layers_Mesh.pdf}}
	\caption{Multilayer problem: The left figure shows the geometry and boundary conditions, 
	and the right figure shows the computational mesh employed in the numerical simulation.}
	\label{fig:layers_Geo}
\end{figure}
%
\begin{figure}[htb!]
  \centering
  \includegraphics[scale=0.3]{./Figures/Ux_vs_y_layers.pdf}
  \caption{Multilayer problem: Variation of $x$-velocity along 
    the vertical centerline of the domain at $x = 0.5$.}
  \label{fig:Layers_Ux_vs_y}
\end{figure}
%
\begin{figure}[htb!]
  \centering
  \subfigure{\includegraphics[scale=0.5]{./Figures/CvsY_0p5.pdf}}
  \subfigure{\includegraphics[scale=0.5]{./Figures/CvsY_1p0.pdf}}
  \subfigure{\includegraphics[scale=0.5]{./Figures/CvsY_1p5.pdf}}
  \caption{Multilayer problem: Variation of the concentration 
    along the vertical line of the domain at $x = 1.0$ for 
    various instances of time $t = 0.5$, $1.0$ and $1.5 \; 
    \mathrm{s}$.} \label{fig:Layers_CvsY}
\end{figure}
%
\begin{figure}[htb!]
  \centering
  \subfigure{ \includegraphics[scale=0.35]{./Figures/RT0_layers_0p2.pdf}}
  \subfigure{ \includegraphics[scale=0.35]{./Figures/VMS_layers_0p2.pdf}}
  \caption{Multilayer problem: Contours of the concentration at time 
    $t = 0.2 \; \mathrm{s}$ using the RT0 formulation (left) and the 
    variational multiscale formulation (right).} \label{fig:Layers_C_contour}
\end{figure}
%
\begin{figure}[htb!]
  \centering
  \includegraphics[scale=0.5]{./Figures/C_vs_time.pdf}
  \caption{Multilayer problem: This figure shows the 
    variation of the total concentration with time. 
    The total concentration is the integral of the 
    concentration field over the entire domain.}
	\label{fig:Layers_CvsTime}
\end{figure}
%
%
\begin{figure}[htb!]
  \centering
  \includegraphics[scale=0.45]{./Figures/VMS_Mass_Balance_Layers.pdf}
  % \subfigure{\includegraphics[scale=0.45]{./Figures/CMB_Mass_Balance_Layers.pdf}}
  \caption{Multilayer problem: This figure shows the contours of the error 
    in the local mass balance under the equal-order variational multiscale 
    formulation.} \label{fig:Layers_Mass_Balance}
\end{figure}
%
\clearpage
%
\begin{figure}[htb!]
	\centering
\subfigure{ \includegraphics[scale=0.55]{./Figures/Inclusion_Geo_New.pdf}}
\subfigure{ \includegraphics[scale=0.52]{./Figures/Inclusion_Mesh.pdf}}
	\caption{Cylinder inclusion: The top figure shows the problem 
          geometry and boundary conditions, and the bottom figure shows 
          the computational mesh used in the numerical simulation.}
	\label{fig:Inclusion_Geo}
\end{figure}
%
\begin{figure}[htb!]
  \centering
  \subfigure{\includegraphics[scale=0.5]{./Figures/RT0_inclusion_V.pdf}}
  \subfigure{  \includegraphics[scale=0.5]{./Figures/VMS_inclusion_V.pdf}}
  \caption{Cylinder inclusion: This figure shows the contours of the 
    magnitude of the velocity using the RT0 formulation (top) and the 
    variational multiscale formulation (bottom) for the case  $k_2 = 
    1\times10^{-3}$.} \label{fig:Vel_x}
\end{figure}
%
\begin{figure}[htb!]
  \centering
  \includegraphics[scale=0.6]{./Figures/Inclusion_Pressure.pdf}
  \caption{Cylinder inclusion: This figure shows the variation 
    of the pressure along $x$-direction at $y = 0$ for the case 
    $k_2 = 1\times10^{-3}$.} \label{fig:Pressure_vs_x}
\end{figure}
%
\begin{figure}[htb!]
  \centering
  \subfigure{ \includegraphics[scale=0.5]{./Figures/Inclusion_Vx_x.pdf}}
  \subfigure{  \includegraphics[scale=0.5]{./Figures/Inclusion_Vx_y.pdf}}
  \caption{Cylinder inclusion: This figure shows the variation of 
    the $x$-velocity along the $x$-direction at $y = 0$ (left), 
    and along the $y$-direction at $x= 0$ (right) for the case 
    $k_2 = 1\times10^{-3}$.}
	\label{fig:Vel_vs_x}
\end{figure}
%
\begin{figure}[htb!]
  \centering
  \subfigure{\includegraphics[scale=0.5]{./Figures/RT0_inclusion_C.pdf}}
  \subfigure{  \includegraphics[scale=0.5]{./Figures/VMS_inclusion_C.pdf}}
  \caption{Cylinder inclusion: This figure shows the contours of the 
    concentration at time $t = 1.5 \; \mathrm{s}$ using the RT0 formulation 
    (top) and the variational multiscale formulation (bottom) for the case 
    $k_2 = 1\times10^{-3}$.} \label{fig:Inclusion_C}
\end{figure}
%
\begin{figure}[htb!]
  \centering
  \includegraphics[scale=0.5]{./Figures/VMS_Inclusion_Mass_Balance.pdf}
  \caption{Cylinder inclusion: This figure shows the contours of the error 
    in the mass balance using the variational multiscale formulation for 
    the case $k_2 = 1\times10^{-7}$.} \label{fig:Inclusion_Mass_Balance}
\end{figure}
%
\begin{figure}[htb!]
  \centering
  \includegraphics[scale=0.5]{./Figures/Inclusion_Ratio.pdf}
  \caption{Cylinder inclusion: The figure shows the variation of 
    the error in the total concentration (which is measured as the 
    difference between the integral of $c$ over the domain at time 
    $t = 2.5 \; \mathrm{s}$ minus the integral of $c$ over the domain 
    at $t = 0.0 \; \mathrm{s}$) with respect to the log of the ratio 
    of permeabilities between the inclusion and the rest of the domain.} 
  \label{fig:Inclusion_Mass_Balance_Ratio}
\end{figure}
%
\begin{figure}[htb!]
  \centering
  \subfigure{ \includegraphics[scale=0.4]{./Figures/leaky_well_domain.pdf}}
  \subfigure{ \includegraphics[scale=0.6]{./Figures/leaky_well_mesh.pdf}}
  \caption{Leaky well: A pictorial description of the problem (top) 
    and the computational mesh used in the numerical simulation 
    (bottom). (Note that a portion of the mesh for the abandoned 
    well is omitted to facilitate plotting.)} 
  \label{fig:LeakyWellDomain}
\end{figure}
%
\newpage
%
\begin{figure}[htb!]
	\centering
 \includegraphics[scale=0.8]{./Figures/leaky_well_v_mags.pdf}
	\caption{Leaky well: velocity magnitude contours using the RT0 
	formulation (top) and the variational multiscale formulation (bottom).}
	\label{fig:LeakyWellVMags}
\end{figure}
%
\newpage
%
\begin{figure}[htb!]
	\centering
 \includegraphics[scale=0.8]{./Figures/leaky_well_p.pdf}
	\caption{Leaky well: pressure contours using the RT0 formulation 
	(top) and the variational multiscale formulation (bottom).}
	\label{fig:LeakyWellP}
\end{figure}
%
%
\begin{figure}[htb!]
  \centering
  \includegraphics[scale=0.8]{./Figures/RT0_leak_contours.pdf}
  \caption{Leaky well: contours of concentration at various times 
    for the RT0 formulation. (Note that a portion of the abandoned 
    well was omitted to facilitate plotting.)} 
  \label{fig:RT0LeakyWellContours}
\end{figure}
%
\newpage
%
\begin{figure}[htb!]
  \centering
  \includegraphics[scale=0.8]{./Figures/VMS_leak_contours.pdf}
  \caption{Leaky well: contours of concentration at various instances 
    of time for the variational multiscale formulation. (Note that a 
    portion of the abandoned well was omitted to facilitate plotting.)}
  \label{fig:VMSLeakyWellContours}
\end{figure}
%

\begin{figure}[htb!]
  \centering
  \includegraphics[scale=0.6]{./Figures/new_leak_rate.pdf}
  \caption{Leaky well: leak rate vs. time measured as the concentration 
    times the mass flux across the opening of the abandoned well into 
   Aquifer B for various values of $\beta$ using the Barus model for 
    viscosity given in equation \eqref{Eqn:FlowTransport_Barus}.}
  \label{fig:LeakRate}
\end{figure}

%
\vspace{5in}
\begin{figure}[htb!]
  \centering
  \includegraphics[scale=0.15]{./Figures/contour_compare.pdf}
  \caption{Leaky well: contours of the concentration at the injection well at $t=0.12$ days for various values of $\beta$ using the Barus model for viscosity given in equation \eqref{Eqn:FlowTransport_Barus} (top) RT0 (bottom) VMS.}
  \label{fig:ContoursCompare}
\end{figure}


==> Sections/S1_PF_Introduction.tex <==
%**********************************;
%                                  ;
%  NAME                            ;
%    S1_PF_Introduction.tex        ;
%                                  ;
%  WRITTEN BY                      ;
%    DZT and KBN                   ;
%                                  ;
%**********************************;
\section{INTRODUCTION}
\label{Sec:S1_Introduction}
In the field of subsurface modeling, choosing the right numerical 
formulation for a particular problem of interest can be a difficult 
choice. There are a number of trade-offs that one must consider. Two 
very important considerations involve accuracy and computational 
efficiency. For problems that involve species transport (reactive 
or not) through a porous domain, artificial production or loss of 
constituents can be detrimental, especially in the case of transport 
of contaminants or pollutants. At the same time, accuracy comes with 
a cost, which manifests in the form of computation time, mesh resolution 
requirements, and/or time step restrictions. An astute analyst must 
balance these tradeoffs such that sufficiently accurate results are 
obtained at a reasonable cost.

In this paper, we compare two popular mixed finite element formulations 
to solve the flow equations in heterogeneous porous media. The two mixed 
formulations are the lowest order Raviart-Thomas formulation (RT0) 
\cite{Raviart_Thomas_MAFEM_1977_p292}, and the variational multiscale 
stabilized formulation (VMS), which has been studied in references 
\cite{Nakshatrala2,Masud4,Nakshatrala_Rajagopal_IJNMF_arxiv_2010,
Nakshatrala_Turner_IJES_2010}. Mixed methods, that treat velocity and pressure as independent variables, as opposed to single field formulations, provide a more accurate representation of the velocity field, but are susceptible to instability engendered by the saddle-point nature of the system of equations \cite{Brezzi}. The VMS element evaluated in this work consists of equal order linear interpolation of the velocity and pressure fields, for which the degrees of freedom live at the node locations. The VMS element achieves stability through the addition of residual based terms to the formulation such that the LBB condition is circumvented. The lowest order Raviart-Thomas finite element formulation (RT0) consists of evaluating fluxes over the midpoint of element edges and constant pressures within the element and is based on an LBB stable finite element space. A schematic of both elements is presented in Figure \ref{fig:Elements}. Both elements are used to solve several realistic engineering problems involving flow and transport in heterogeneous porous media.

The pursuit of stable, locally conservative finite element formulations has received substantial attention (for examples see \cite{Brezzi_Douglas_Marini_NumerMath_1985_v88_p217, Barrenechea, Arbogast_Huang_Russel_Preprint} among many others). In addition, a number of comparisons have been made between various formulations (for example, see \cite{Mazzia, Kippe, Durlofsky_WRR_1994_v30_p965}), Of particular interest is the work presented in \cite{Durlofsky_WRR_1994_v30_p965} that showed a computational efficiency advantage for control volume approaches vs. mixed methods for problems with only moderate heterogeneity.

It is well known that the VMS element, which is based on a Galerkin formulation is not locally mass conserving (without additional sophistication being built into the algorithm as in \cite{Hughes_Engel_Mazzei_Larson_JCP_2000_v163_p467,Dogrul_Kadir_JHE_2006_v132_p1206}), but the degree to which a realistic simulation will suffer due to this shortcoming of the VMS element is not well documented. Additionally, although the RT0 element is locally conservative, it has only been shown viable for triangular or tetrahedral elements (quadrilateral variants of this method do not pass the patch test). In the context of heterogeneous materials, this work aims, to evaluate the strengths and weaknesses of either approach for problems with highly varying material permeability and predominantly open flow boundary conditions. The results have applications in subsurface simulations for which the far-field boundary is typically described with some type of pressure boundary condition. 

%================================================;
%  Subsection: Main contributions of this paper  ;
%================================================;
\subsection{Main contributions of this paper}
One of the main goals of this paper is to assess the performance 
of the variational multiscale formulation with respect to local 
(or element) mass balance using a coupled flow-transport model. 
The assessment is performed by comparing the variational multiscale 
formulation with the lowest-order Raviart-Thomas formulation, which 
possesses the local mass balance property. We also take into account 
the dependence of viscosity on the pressure, which is the case with 
most organic liquids and supercritical carbon-dioxide. Using Barus 
model (in which the viscosity varies exponentially with respect to 
pressure), we study the affect of the dependence of viscosity of 
pressure on the error in the local mass balance under the variational 
multiscale formulation. Using canonical problems, we also compare 
the performance of the variational multiscale formulation and the lowest 
order Raviart-Thomas formulation with respect to memory storage, time 
for assembling matrices, and total CPU time. 

%=========================================;
%  Subsection: Organization of the paper  ;
%=========================================;
\subsection{Organization of the paper}
The remainder of this paper is organized as follows. In Section 
\ref{Sec:S2_PF_Governing_equations}, we present a coupled flow-transport 
mathematical model. In Section \ref{Sec:S3_Weak_formulations}, we present 
weak formulations to solve both flow and transport problems. For the flow 
problem, we consider the variational multiscale formulation and the lowest-order 
Raviart-Thomas formulation. In Section \ref{Sec:S4_Numerical_results}, we present 
numerical results for flow and transport for three canonical problems: a stratified 
set of layers with differing permeabilities, a cylindrical inclusion of high 
permeability in a domain of lower permeability, and a leaky well scenario where 
a storage aquifer leaks the injected constituent through an abandoned well. In 
Section \ref{Sec:S5_Conclusions}, we conclude with a summary of the important 
research findings of this paper. 


==> Sections/S2_PF_Governing_Equations.tex <==
%***********************************************************;
%                     
%    Governing_Equations generated by ManuscrtipMaker.sh
%
%    Author: dzturne 
%
%    Date: Mon Nov 23 07:14:03 MST 2009 
%
%************************************************
\section{A COUPLED FLOW-TRANSPORT MATHEMATICAL MODEL}
\label{Sec:S2_PF_Governing_equations}
Consider the transport of a chemical species in a rigid porous medium 
(that is, the deformation of the porous solid is neglected). We shall 
assume that the porous medium is fully saturated with a (moving) fluid. 
Herein, we consider modified Darcy equation for the flow problem which 
(as the name suggests) is a modification to the standard Darcy equation 
\cite{Darcy_1856}. This model takes into account the dependence of viscosity 
on the pressure. The fluid is still assumed to be incompressible. The 
transport model consists of transient advection-diffusion equation wherein 
the advection velocity is given by the flow problem. 

%========================================================;
%  Subsection: Governing equations for the flow problem  ;
%========================================================;
\subsection{Governing equations for the flow problem}
Let $\Omega$ be a bounded open domain, and $\Gamma$ be its piecewise 
smooth boundary ($\Gamma := \bar{\Omega} - \Omega$, where $\bar{\Omega}$ 
is the set closure of $\Omega$). A spatial point is denoted by $\boldsymbol{x} 
\in \Omega$. The gradient and divergence operators with respect to $\boldsymbol{x}$ 
are, respectively, denoted by $\mathrm{grad}[\cdot]$ and $\mathrm{div}[\cdot]$. 
Let $p:\Omega \rightarrow \mathbb{R}$ denote the pressure, and the velocity 
field is denoted by $\boldsymbol{v}:\Omega \rightarrow \mathbb{R}^{nd}$, 
where ``$nd$'' is the number of spatial dimensions. We denote the density 
by $\rho $, the permeability by $k(\boldsymbol{x})$, and the coefficient 
of viscosity by $\mu$. We consider the following expressions for the 
dependence of viscosity on the pressure:
%-------------------------------------------------;
%  Equation: Dependence of viscosity on pressure  ;
%-------------------------------------------------;
\begin{subequations} 
  \begin{align}
    \label{Eqn:FlowTransport_constant}
    \mu(p) &= \mu_0 \\
    %
    \label{Eqn:FlowTransport_Barus}
    \mu(p) &= \mu_0 \exp[\beta p]
  \end{align}
\end{subequations}
%
where $\mu_0 > 0$ is the coefficient of viscosity at a reference pressure (e.g., 
at the atmospheric pressure), and $\beta \geq 0$ is a constant. Equation 
\eqref{Eqn:FlowTransport_constant} assumes the viscosity is constant, 
which is the case in the standard Darcy flow model \cite{Darcy_1856}. 
Equation \eqref{Eqn:FlowTransport_Barus} is commonly referred to as 
Barus formula \cite{Barus_AJS_1893_v45_p87}.

We write the governing equations for the flow in first-order form 
(or mixed form) in which the velocity and pressure are treated as 
independent variables. The governing equations for the flow problem 
can be written as follows: 
%------------------------------------------;
%  Equation: Governing equations for flow  ;
%------------------------------------------;
\begin{subequations}
  \begin{align}
    \label{Eqn:Forchheimer}
    \frac{\mu(p)}{k} \boldsymbol{v} + \mathrm{grad}[p] &= \rho 
    \boldsymbol{b}(\boldsymbol{x}) \qquad \mbox{in} \; \Omega \\
    % 
    \label{Eqn:AD_DirichletBC}
    \mathrm{div}[\boldsymbol{v}] &= \phi(\boldsymbol{x}) \qquad 
    \mbox{in} \; \Omega \\
    % 
    \label{Eqn:AD_NeumannBC}
    \boldsymbol{v}(\boldsymbol{x}) \cdot \boldsymbol{n}(\boldsymbol{x}) 
    &= \psi(\boldsymbol{x}) \qquad \mbox{on} \; \Gamma 
  \end{align}
\end{subequations}
%
where $\boldsymbol{b}(\boldsymbol{x})$ is the specific body force, 
$\phi(\boldsymbol{x})$ is the prescribed volumetric flow rate, $\psi
(\boldsymbol{x})$ is the prescribed normal component of the velocity 
on the boundary, and $\boldsymbol{n}(\boldsymbol{x})$ is the unit 
outward normal vector to $\Gamma$. Note that for a given $\Omega$ 
(and hence for a given $\Gamma$), $\phi(\boldsymbol{x})$ and $\psi
(\boldsymbol{x})$ are not independent of each other, and they need 
to satisfy the following compatibility condition: 
%-------------------------------------;
%  Equation: Compatibility condition  ;
%-------------------------------------;
\begin{align}
  \int_{\Omega} \phi(\boldsymbol{x}) \; \mathrm{d} \Omega 
  &= \int_{\Gamma} \psi(\boldsymbol{x}) \; \mathrm{d} \Gamma
\end{align}
%
Since we have prescribed only the normal component of the velocity 
on the whole boundary, one need to enforce one more condition to 
obtain unique solution in the pressure field. This is typically 
achieved by meeting the following condition: 
\begin{align}
  \int_{\Omega} p(\boldsymbol{x}) \; \mathrm{d} \Omega = 0
\end{align}
%
Another way to achieve uniqueness in the pressure field is to 
prescribe the pressure at a point to fix the datum, which is 
computationally the most convenient and is employed in this 
paper. In pressure-driven flows, there is no need to enforce 
additional conditions for uniqueness as the pressure is 
prescribed on a set of non-zero measure on the boundary. 

%===========================================================;
%  Subsection: Governing equations for the transport model  ;
%===========================================================;
\subsection{Governing equations for the transport problem}
Let $c(\boldsymbol{x},t)$ denote the concentration, and $\mathcal{I}$ 
denote the time interval of interest. The boundary $\Gamma$ is divided 
into two complementary parts $\Gamma^{\mathrm{D}}_c$ and 
$\Gamma^{\mathrm{N}}_c$. $\Gamma^{\mathrm{D}}_c$ is that part of the 
boundary on which Dirichlet boundary condition is prescribed (that is, 
the concentration is prescribed), and $\Gamma^{\mathrm{N}}_c$ is that 
part of the boundary on which the Neumann boundary condition is 
prescribed. The transport problem is to find $c(\boldsymbol{x},t)$ 
by solving the following initial boundary value problem: 
%--------------------------------------------------------------------;
%  Equation: Governing equations of the advection-diffusion problem  ;
%--------------------------------------------------------------------;
\begin{subequations}
  \begin{align}
    \label{Eqn:AD_Equilibrium}
    \frac{\partial c}{\partial t} + \boldsymbol{v}(\boldsymbol{x}) \cdot 
    \mathrm{grad}[c] - \mathrm{div}\left[D \; \mathrm{grad}[c]\right] &= 
    f(\boldsymbol{x},t) \qquad \; \;  \ \mbox{in}  \quad \Omega \times 
    \mathcal{I} \\
    % 
    \label{Eqn:AD_DirichletBC}
    c(\boldsymbol{x},t) &= c^{\mathrm{p}}(\boldsymbol{x},t) 
    \qquad \; \mbox{on} \quad \Gamma^{\mathrm{D}}_c \times \mathcal{I} \\
    % 
    \label{Eqn:AD_NeumannBC}
    D \; \mathrm{grad}[c]\cdot \boldsymbol{n}(\boldsymbol{x}) &= 
    t^{\mathrm{p}}(\boldsymbol{x},t) \qquad \; \; \; \mbox{on} \quad 
    \Gamma^{\mathrm{N}}_c \times \mathcal{I}
    % 
  \end{align}
\end{subequations}
%
where $D$ is the constant diffusivity of the species, $c^{\mathrm{p}}(\boldsymbol{x},t)$ 
is the prescribed Dirichlet boundary condition on concentration, $t^{\mathrm{p}}
(\boldsymbol{x},t)$ is the prescribed flux, $f(\boldsymbol{x},t)$ is the volumetric 
source term, and $\boldsymbol{n}(\boldsymbol{x})$ is the unit outward normal 
vector to $\Gamma$. 

==> Sections/S3_PF_Weak_formulations.tex <==
%***********************************************************;
%                     
%    Governing_Equations generated by ManuscrtipMaker.sh
%
%    Author: dzturne 
%
%    Date: Mon Nov 23 07:14:03 MST 2009 
%
%************************************************
\section{WEAK FORMULATIONS}
\label{Sec:S3_Weak_formulations}
In this section, we present two mixed formulations for the flow problem, and 
a single-field formulation for solving the transport problem. The first mixed 
formulation is based on the Raviart-Thomas spaces, and the other is the 
variational multiscale formulation presented in Reference 
\cite{Nakshatrala_Turner_IJES_2010}.

%======================================================;
%  Subsection: Weak formulations for the flow problem  ;
%======================================================;
\subsection{Weak mixed formulations for the flow problem}
Let the weighting function corresponding to the velocity be denoted 
by $\boldsymbol{w}(\boldsymbol{x})$, and the weighting function 
corresponding to the pressure be denoted by $q(\boldsymbol{x})$. 
The relevant function spaces for the velocity and the corresponding 
weighting function are, respectively, defined as follows:  
%------------------------------------------------;
%  Equation: Function spaces for velocity and w  ;
%------------------------------------------------;
\begin{subequations}
  \begin{align}
    % ---------;
    %  v space ;
    % ---------;
    \label{Eqn:Function_Space_for_v}
    \mathcal{V} &:= \{\boldsymbol{v}(\boldsymbol{x}) | \boldsymbol{v}
    (\boldsymbol{x}) \in \left(L_2(\Omega)\right)^{nd}, \mathrm{div}
    [\boldsymbol{v}] \in L_2(\Omega), \mathrm{trace}[\boldsymbol{v} 
    \cdot \boldsymbol{n}] = \psi(\boldsymbol{x}) \in H^{-1/2}(\Gamma) \} \\
    %----------;
    %  w space ;
    %----------;
    \mathcal{W} &:= \{\boldsymbol{w}(\boldsymbol{x}) | \boldsymbol{w}
    (\boldsymbol{x}) \in \left(L_2(\Omega)\right)^{nd}, \mathrm{div}
    [\boldsymbol{w}] \in L_2(\Omega), \mathrm{trace}[\boldsymbol{w} 
    \cdot \boldsymbol{n}] = 0 \; \mathrm{on} \; \Gamma \}
    % 
  \end{align}
\end{subequations}
% 
where $L_2(\Omega)$ is the space of square integrable functions, 
$\mathrm{trace}[\cdot]$ is the standard trace operator used in functional 
analysis \cite{Evans_PDE}, and $H^{-1/2}(\Gamma)$ is the dual space 
of $H^{1/2}(\Gamma)$. In the classical mixed formulation, the function 
space for the pressure and its corresponding weighting function is 
defined as follows:
% -----------------------------------;
%  p space for Galerkin formulation  ;
% -----------------------------------;
\begin{align}
  \label{Eqn:Function_Space_for_p}
  \mathcal{P} &:= \{p(\boldsymbol{x}) | p(\boldsymbol{x}) \in 
  L_2(\Omega) , \int_{\Omega} p(\boldsymbol{x}) \; \mathrm{d} 
  \Omega = 0 \}
\end{align}
%
In the variational multiscale formulation, the function space for 
the pressure and its corresponding weighting function is defined 
as follows: 
%-------------------------------;
%  p space for VMS formulation  ;
%-------------------------------;
\begin{align}
  \label{Eqn:Function_Space_for_p_HVM}
  \bar{\mathcal{P}} &:= \{p(\boldsymbol{x}) | p(\boldsymbol{x}) \in 
  H^1(\Omega) , \int_{\Omega} p(\boldsymbol{x}) \; \mathrm{d} \Omega = 0 \}
\end{align}
%
where $H^{1}(\Omega)$ is a standard Sobolev space \cite{Brezzi_Fortin}. 
%
We shall employ the following notation for the standard $L^2$ inner product: 
\begin{align}
(\boldsymbol{a}; 
\boldsymbol{b})  = \int_{\Omega} \boldsymbol{a} \cdot \boldsymbol{b} \; \mathrm{d}
\Omega 
\end{align}

%=====================================================================;
%  Subsection: Classical mixed formulation and Raviart-Thomas spaces  ;
%=====================================================================;
\subsubsection{Classical mixed formulation and Raviart-Thomas spaces}
The classical mixed formulation reads: Find $\boldsymbol{v}(\boldsymbol{x}) 
\in \mathcal{V}$ and $p(\boldsymbol{x}) \in \mathcal{P}$ such that we have 
%-----------------------------------------;
%  Equation: Classical mixed formulation  ;
%-----------------------------------------; 
\begin{align}
  \label{Eqn:WeakRT0} 
  (\boldsymbol{w};  \frac{\mu} {k} \boldsymbol{v}) - 
  (\mathrm{div}[\boldsymbol{v}];p) - (q;\mathrm{div}
  [\boldsymbol{v}] - \phi) = (\boldsymbol{w}; 
  \rho \boldsymbol{b}) \quad \forall \boldsymbol{w}
  (\boldsymbol{x}) \in \mathcal{W}, \; q(\boldsymbol{x}) 
  \in \mathcal{P}
\end{align}
%
Let $\mathcal{V}_{h}$, $\mathcal{W}_{h}$ and $\mathcal{P}_{h}$ are, 
respectively, appropriate subspaces of $\mathcal{V}$, $\mathcal{W}$ 
and $\mathcal{P}$. A (conforming) finite element formulation reads: 
Find $\boldsymbol{v}_{h}(\boldsymbol{x}) \in \mathcal{V}_{h}$ and 
$p_{h}(\boldsymbol{x}) \in \mathcal{P}_{h}$ such that we have 
%----------------------------------------;
%  Equation: Finite element formulation  ;
%----------------------------------------;
\begin{align}
  \label{Eqn:WeakRT0_finite_dimensional} 
  (\boldsymbol{w}_{h};  \frac{\mu} {k} \boldsymbol{v}_{h}) - 
  (\mathrm{div}[\boldsymbol{v}_{h}];p_{h}) - (q_{h};
  \mathrm{div}[\boldsymbol{v}_h] - \phi) &= (\boldsymbol{w}_{h}; 
  \rho \boldsymbol{b})   \quad \forall \boldsymbol{w}_{h}
  (\boldsymbol{x}) \in \mathcal{W}_{h}, \; q_{h}(\boldsymbol{x}) 
  \in \mathcal{P}_{h}
\end{align}
%
It is well-known that inclusions $\mathcal{V}_{h} \subset \mathcal{V}$, 
$\mathcal{W}_{h} \subset \mathcal{W}$ and $\mathcal{P}_{h} \subset 
\mathcal{P}$ do not insure stable numerical results. Specifically, not 
all combinations of interpolation functions for the velocity and pressure 
are stable. A mathematical theory concerning the stability of formulations 
and choice of appropriate finite dimensional spaces is given by 
Ladyzhenskaya-Babu\v ska-Brezzi (LBB) stability condition 
\cite{Ladyzhenskaya_Mathematical_Physics,
Babuska_NumerMath_1971_v16_p322,Brezzi_Fortin}. 

In the literature one can find two different ways of obtaining stable 
results: circumventing the LBB condition and satisfying the LBB condition 
\cite{Franca_Hughes_CMAME_1988_v69_p89}. In the former category, 
stabilization terms are added to the classical mixed formulation to achieve 
stability. Many stabilized formulations fall in the former category (e.g., 
references \cite{Masud_Hughes_CMAME_2002_v191_p4341,
Nakshatrala_Turner_Hjelmstad_Masud_CMAME_2006_v195_p4036,
Nakshatrala_Turner_IJES_2010}). Some of the approaches 
in the later category are Raviart-Thomas spaces \cite{Raviart_Thomas_MAFEM_1977_p292}, 
Brezzi-Douglas-Marini spaces \cite{Brezzi_Douglas_Marini_NumerMath_1985_v47_p217}. 
In this paper, for the flow problem, we shall consider the lowest order Raviart-Thomas spaces 
and the variational multiscale formulation. 

We now present the lowest-order Raviart-Thomas triangular spaces. 
Let $\mathcal{T}_h$ be triangulation on $\Omega$. The lowest order 
finite dimensional subspaces on triangles are defined as follows:
 %---------;
  % v space RT0;
  %---------;
\begin{subequations}
\begin{align}
  \label{Eqn:Function_Space_for_v_RT0}
  \mathcal{V}_h &:= \{ \boldsymbol{v} = (v^{(1)},v^{(2)}) \; | \; v_{K}^{(1)} = a_{K} + b_{K} x, 
  v_{K}^{(2)} = c_{K} + b_{K} y ; a_{K}, b_{K}, c_{K} \in \mathbb{R}; K \in  \mathcal{T}_h \} \\
 % \label{Eqn:Function_Space_for_w_RT0}
%\textcolor{red}{ 
\mathcal{W}_h &:= \{ \boldsymbol{w} = (w^{(1)},w^{(2)}) \; | \; w_{K}^{(1)} = a_{K} + b_{K} x, 
w_{K}^{(2)} = c_{K} + b_{K} y ; a_{K}, b_{K}, c_{K} \in \mathbb{R}; K \in  \mathcal{T}_h \} \\
  \label{Eqn:Function_Space_for_p_RT0}
  \mathcal{P}_h &:= \{ p(\boldsymbol{x}) \; | \; p(\boldsymbol{x}) = 
  \mathrm{a \; constant \; on \; each \; triangle \;} K \in  \mathcal{T}_h \}
\end{align}
\end{subequations}

%=====================================================;
%  Subsubsection: Variational multiscale formulation  ;
%=====================================================;
\subsubsection{Variational multiscale formulation}
A stabilized formulation based on the variational multiscale formalism 
can be written as follows \cite{Nakshatrala_Rajagopal_IJNMF_arxiv_2010}: 
Find $\boldsymbol{v}(\boldsymbol{x}) \in \mathcal{V}$ and $p(\boldsymbol{x}) 
\in \mathcal{Q}$ such that we have 
%------------------------------------------------;
%  Equation: Variational multiscale formulation  ;
%------------------------------------------------;
\begin{align}
  \label{Eqn:WeakVMS}  
  (\boldsymbol{w};\frac{\mu}{k}\boldsymbol{v}) &- (\mathrm{div}
  [\boldsymbol{w}];p) - (q;\mathrm{div}[\boldsymbol{v}] - \phi) 
  - (\boldsymbol{w}; \rho \boldsymbol{b}) \nonumber \\ 
  %
  &- \frac{1}{2}\left(\frac{\mu}{k}\boldsymbol{w} + \mathrm{grad}[q];
    \frac{k}{\mu}(\frac{\mu}{k} \boldsymbol{v} + \mathrm{grad}[p] - 
    \rho \boldsymbol{b})\right) = 0 \quad \forall \boldsymbol{w}
  (\boldsymbol{x}) \in \mathcal{W}, \; q(\boldsymbol{x}) \in \mathcal{Q}
\end{align}
%----------------------------------------;
%  Remark: Remark about HVM formulation  ;
%----------------------------------------;
\begin{remark}
  If the coefficient of viscosity is constant the formulation presented 
  in Reference \cite{Nakshatrala_Rajagopal_IJNMF_arxiv_2010} is same as 
  the formulation discussed in References \cite{Masud_Hughes_CMAME_2002_v191_p4341,
    Nakshatrala_Turner_Hjelmstad_Masud_CMAME_2006_v195_p4036}.
\end{remark}

\subsubsection{Pressure boundary conditions}
It is well-known that strongly enforced outflow boundary conditions can 
produce spurious oscillations in the solution \cite{Engelman, Bazilevs, 
SaniBCs, SaniBCs2}. Let $\Gamma_p$ denote that part of the boundary 
on which the pressure is prescribed, and let $\Gamma_v$ be that part of 
the boundary on which the normal component of the velocity is prescribed.  
(As usual, for well-posedness we have $\Gamma_v \cup \Gamma_p = 
\Gamma$ and $\Gamma_v \cap \Gamma_p = \emptyset$.)
%
A simple procedure for enforcing the pressure boundary condition is to 
replace the term $-(\mathrm{div}[\boldsymbol{w}];p)$ with the terms 
\begin{align*}
-(\mathrm{div}[\boldsymbol{w};p) + (\boldsymbol{w}\cdot\boldsymbol{n};
p_0)_{\Gamma_p}
\end{align*}
%
in the mathematical statements \eqref{Eqn:WeakRT0} and \eqref{Eqn:WeakVMS} 
and subsequent steps. In such cases, the function spaces for the velocity and 
corresponding weighting function will be modified as follows:
%------------------------------------------------;
%  Equation: Function spaces for velocity and w  ;
%------------------------------------------------;
  \begin{align*}
    % ---------;
    %  v space ;
    % ---------;
    \mathcal{V} &:= \{\boldsymbol{v}(\boldsymbol{x}) | \boldsymbol{v}
    (\boldsymbol{x}) \in \left(L_2(\Omega)\right)^{nd}, \mathrm{div}
    [\boldsymbol{v}] \in L_2(\Omega), \mathrm{trace}[\boldsymbol{v} 
    \cdot \boldsymbol{n}] = \psi(\boldsymbol{x}) \in H^{-1/2}(\Gamma_v) \} \\
    %----------;
    %  w space ;
    %----------;
    \mathcal{W} &:= \{\boldsymbol{w}(\boldsymbol{x}) | \boldsymbol{w}
    (\boldsymbol{x}) \in \left(L_2(\Omega)\right)^{nd}, \mathrm{div}
    [\boldsymbol{w}] \in L_2(\Omega), \mathrm{trace}[\boldsymbol{w} 
    \cdot \boldsymbol{n}] = 0 \; \mathrm{on} \; \Gamma_v \}
    % 
  \end{align*}

\begin{table}[htb!]
  \caption{Summary of formulation properties \label{table:FormProps}}
  \centering
  \begin{tabular}{l c c c c c} \hline
                 & Global       & Local (element)  & Convergence    & Convergence    \\
    Formulation  & mass balance & mass balance     & rate velocity  & rate pressure  \\ \hline
    RT0          & Yes          & Yes              & 1.0            &  1.0           \\
    VMS          & Yes          & No               & 2.0            &  1.0           \\ \hline
  \end{tabular}
\end{table}

%============================================;
%  Subsection: Weak formulation for the transport problem  ;
%============================================;
\subsection{Weak formulation for the transport problem}
We employ the standard single-field formulation to solve the transport equations, 
which is based on the Galerkin principle. Let us denote the weighting function 
corresponding to the concentration as $w^{c}(\boldsymbol{x})$. We shall define 
the following function spaces for the concentration and the corresponding weighting 
function:
\begin{subequations}
\begin{align}
  %---------;
  % v space ;
  %---------;
  \label{Eqn:AD_Function_Space_for_u}
  \mathcal{C}_{t} &:= \{c(\boldsymbol{x},t)  \; \big| \; c(\boldsymbol{x},t) \in H^{1}(\Omega),
  c(\boldsymbol{x},t) = c^{\mathrm{p}}(\boldsymbol{x},t) \; \mathrm{on} \; \Gamma^{\mathrm{D}}_c \} \\
  %---------;
  % w space ;
  %---------;
  \label{Eqn:AD_Function_Space_for_w}
  \mathcal{W}^c &:= \{w^{c}(\boldsymbol{x})  \; \big| \; w^{c}(\boldsymbol{x}) \in H^{1}(\Omega),
  w^{c}(\boldsymbol{x}) = 0 \; \mathrm{on} \; \Gamma^{\mathrm{D}}_c \} 
  %
\end{align}
\end{subequations}
%
The weak form can be expressed as: Find $c(\boldsymbol{x},t) \in \mathcal{C}_t$ such that 
%-----------------------------------;
%  Equation: Classical formulation  ;
%-----------------------------------;  
\begin{align}
  \label{Eqn:AD_Classical_Functional}
  (w; \frac{\partial c}{\partial t}) + ( w^{c} ; \boldsymbol{v} \cdot \mathrm{grad}[c] ) 
  + (\mathrm{grad}[w^{c}] ; D \; \mathrm{grad}[c] ) =
 ( w^{c} ; f ) + ( w^{c}; t^{\mathrm{p}})_{\Gamma^{\mathrm{D}}_c}
  \quad \forall w^{c}(\boldsymbol{x}) \in \mathcal{W}^c
\end{align}

\begin{remark}
In addition to the local mass balance error associated with the flow problem, there will also be an error associated with the transport problem. Since the focus of this work is on the characteristics of the flow problem we are assuming that the transport error is the same for the velocity field generated by both the RT0 and VMS formulations. 
\end{remark}

==> Sections/S5_PF_Conclusions.tex <==
%*******************************************;
%                                           ;
%  NAME                                     ;
%    S5_PF_Conclusions.tex                  ; 
%                                           ;
%  WRITTEN BY                               ;
%    Daniel Turner, Kalyana Nakshatrala     ;
%                                           ;
%*******************************************;
\section{CONCLUSIONS}
\label{Sec:S5_Conclusions}
The results of this study reveal several interesting features 
of the lowest Raviart-Thomas and the variational multiscale 
formulation when used to model flow through heterogeneous 
porous media. Although the equal-order interpolation for 
the velocity and pressure under the variational multiscale 
formulation does not exhibit local (or element) mass balance. 
In addition, the formulation also shows oscillations in the 
velocity field when the primary flow direction is tangential 
to jumps in permeability, for some transport problems, the 
resulting concentration field is only marginally affected. 
%
For the multilayer problem and the cylinder inclusion problem, 
the mass conservation error produced by using the variational 
multiscale formulation is less than 2\%. On the other hand, 
for transport problems similar to the leaky well problem, the 
equal-order interpolation under the variational multiscale 
formulation not only shows a substantial error in the 
concentration, but also under-predicts the leak rate, 
which is undesirable from a design perspective. For the 
leaky well problem, the leak rate was under-predicted by 
roughly 10\% by the variational multiscale formulation. 
The results of this study also reveal that for small to 
moderately sized problems, the increased size of the linear 
system of equations for the RT0 formulation is offset by a 
reduced computation time. For large problems, this advantage 
diminishes. In general, these results give some perspective 
on the computational cost associated with using a locally 
mass conserving element, and the accuracy cost of using a 
stabilized element.
